CultureLLM: Incorporating Cultural Differences into Large Language Models

Large language models (LLMs) are reported to be partial to certain cultures owing to the training data dominance from the English corpora. Since multilingual cultural data are often expensive to collect, existing efforts handle this by prompt engineering or culture-specific pre-training. However, they might overlook the knowledge deficiency of low-resource culture and require extensive computing resources. In this paper, we propose CultureLLM, a cost-effective solution to incorporate cultural differences into LLMs. CultureLLM adopts World Value Survey (WVS) as seed data and generates semantically equivalent training data via the proposed semantic data augmentation. Using only 50 seed samples from WVS with augmented data, we fine-tune culture-specific LLMs and one unified model (CultureLLM-One) for 9 cultures covering rich and low-resource languages. Extensive experiments on 60 culture-related datasets demonstrate that CultureLLM significantly outperforms various counterparts such as GPT-3.5 (by 8.1%) and Gemini Pro (by 9.5%) with comparable performance to GPT-4 or even better. Our human study shows that the generated samples are semantically equivalent to the original samples, providing an effective solution for LLMs augmentation. Code is released at https://github.com/Scarelette/CultureLLM.

==> old_table/tb-datasets.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[]
\label{tb-datasets}
\caption{Details on our evaluation tasks and datasets. There are $59$ testsets covering $9$ languages. We list both the name and the size of test sets. For instance, ``OffensEval2020 (2000)~\citeyearpar{zampieri2020semeval}'' denotes that there are 2000 test samples in the dataset OffensEval2020.}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|c|p{18cm}|c}
\toprule
\method  & Culture & Country & Task \& Dataset & \#Sample \\ \midrule
\method-Ar & Arabic  & Middle East & \makecell{\textit{Offensive language detection:} OffensEval2020~\citeyearpar{zampieri2020semeval}, OSACT4 (1000)~\citeyearpar{husain2005osact4}, Multi-Platform (1000)~\citeyearpar{chowdhury2020multi}, and OSACT5 (2541)~\citeyearpar{mubarak2022overview}. \\\textit{Hate detection:} OSACT4 (1000)~\citeyearpar{husain2005osact4}, Multi-Platform 
(675)~\citeyearpar{chowdhury2020multi}, OSACT5 (2541)~\citeyearpar{mubarak2022overview}, and OSACT5\_finegrained (2541)~\citeyearpar{mubarak2022overview}. \\\textit{Spam detection:} ASHT (1000)~\citeyearpar{kaddoura2024dataset}. \\\textit{Vulgar detection:} Multi-Platform (675)~\citeyearpar{chowdhury2020multi}}    & xxx                    
% & \makecell{OSACT4 \\(1000)~\citeyearpar{husain2005osact4}}                                        & \makecell{Multi-Platform\\(1000)~\citeyearpar{chowdhury2020multi}}                                    & \makecell{OSACT5\\(2541)~\citeyearpar{mubarak2022overview} }                                             \\
%   &  &   & Hate detect                  & \makecell{OSACT4\\(1000)~\citeyearpar{husain2005osact4}}                                      & \makecell{Multi-Platform \\(675)~\citeyearpar{chowdhury2020multi}}                                   & \makecell{OSACT5\\(2541)~\citeyearpar{mubarak2022overview}}                                              &                                  \makecell{OSACT5\_finegrained\\(2541)~\citeyearpar{mubarak2022overview}}                            \\
%  &  &  & Spam detect                  & \makecell{ASHT\\(1000)~\citeyearpar{kaddoura2024dataset}}           &                                                     &                                                         &                                                           \\
%  &  & & Vulgar detect                & \makecell{Multi-Platform\\(675)~\citeyearpar{chowdhury2020multi} }                             &                                                       &                                                         &                                                           \\ \midrule
% \multirow{8}{*}{\method-Bn} & \multirow{8}{*}{Bengali}  & \multirow{8}{*}{Bangladesh}  & Offensive detect             & \makecell{TRAC2020 Task1\\(1000)~\citeyearpar{trac2-dataset}}                      & \makecell{TRAC2020 Task2\\(1000)~\citeyearpar{trac2-dataset}}                            & \makecell{BAD\\(1000)~\citeyearpar{sharif2022tackling}}                                               &                                                           \\
%             &  &   & Hate detect                  & \makecell{Hate Speech\\(1000)~\citeyearpar{romim2021hate}}                               &                                                       &                                                         &                                                           \\
%             &  &   & Threat detect                & \makecell{BACD\\(1000)~\citeyearpar{Bangla-Abusive-Comment-Dataset}}           &                                                       &                                                         &                                                           \\
%             &  &   & Bias detect                 & \makecell{BACD\\(1000)~\citeyearpar{Bangla-Abusive-Comment-Dataset}}            &                                                       &                                                         &                                                           \\ \midrule
% \multirow{6}{*}{\method-Zh} & \multirow{6}{*}{Chinese}  & \multirow{6}{*}{China}   & Spam detect                  & \makecell{CCS\\(1000)~\citeyearpar{jiang2019detect}}                                       &                                                       &                                                         &                                                           \\
%             &  &   & Bias detect                 & \makecell{CDial-Bias\\(1000)~\citeyearpar{zhou2022towards}}                               &                                                       &                                                         &                                                           \\
%             &  &   & Stance detect               & \makecell{CValues\\(1712)~\citeyearpar{xu2023cvalues}}                                   &                                                       &                                                         &                                                           \\ \midrule
% \multirow{8}{*}{\method-En} & \multirow{8}{*}{English}  & \multirow{8}{*}{United States}    & Offensive detect             & \makecell{SOLID\\(1000)~\citeyearpar{rosenthal2020solid}}                                     &                                                       &                                                         &                                                           \\
%             &  &   & Hate detect                  & \makecell{MLMA\\(1000)~\citeyearpar{ousidhoum-etal-multilingual-hate-speech-2019}}                                      &  \makecell{HOF\\(1000)~\citeyearpar{hateoffensive}} &                                                         &                                                           \\
%             &  &   & Threat detect               & \makecell{JMT\\(1000)~\citeyearpar{Jigsaw-Multilingual-Toxicity}}              &                                                       &                                                         &                                                           \\
%             &  &   & Toxicity detect             & \makecell{MLMA\\(1000)~\citeyearpar{ousidhoum-etal-multilingual-hate-speech-2019}}                                      & \makecell{JMT\\(1000)~\citeyearpar{Jigsaw-Multilingual-Toxicity}}                    &                                                         &                                                           \\ \midrule
% \multirow{4}{*}{\method-De} & \multirow{4}{*}{German}  & \multirow{4}{*}{Germany}    & Offensive detect             & \makecell{GermEval2018\\(3531)~\citeyearpar{wiegand2018overview}}                              &                                                       &                                                         &                                                           \\
%             &  &   & Hate detect                  & \makecell{IWG\_1\\(469)~\citeyearpar{ross2016hatespeech}}       & \makecell{IWG\_2\\(469)~\citeyearpar{ross2016hatespeech}}             & \makecell{HASOC2020\\(850)~\citeyearpar{HASOC2020}}                                          &  \makecell{multilingual-hatecheck\\(1000)~\citeyearpar{rottger2022multilingual}} \\ \midrule
% \multirow{4}{*}{\method-Ko} & \multirow{4}{*}{Korean}  & \multirow{4}{*}{South Korea}     & Hate detect                  & \makecell{KMHaS\\(1000)~\citeyearpar{lee-etal-2022-k}}       &  \makecell{hateSpeech\\(1000)~\citeyearpar{moon-etal-2020-beep}} &  \makecell{HateSpeech2\\(1000)~\citeyearpar{Korean-HateSpeech-dataset}} &                                                           \\
%             &  &   & Abusive detect              & \makecell{AbuseEval\\(1000)~\citeyearpar{caselli2020feel}}                                 & \makecell{CADD\\(1000)~\citeyearpar{song2021large}}                                            & \makecell{Waseem\\(1000)~\citeyearpar{waseem2016hateful}}                                            &                                                           \\ \midrule
% \multirow{6}{*}{\method-Pt} & \multirow{6}{*}{Portuguese}  & \multirow{6}{*}{Brazil}  & Offensive detect             & \makecell{OffComBR\\(1250)~\citeyearpar{Pelle2017}}                                  & \makecell{HateBR\\(1000)~\citeyearpar{vargas-etal-2022-hatebr}}                                          &                                                         &                                                           \\
%             &  &   & Bias detect                 & \makecell{ToLD-Br\\(1000)~\citeyearpar{leite2020toxic}}                                   & \makecell{ToLD-Br\\(1000)~\citeyearpar{leite2020toxic}}                                         &                                                         &                                                           \\
%             &  &   & Abusive detect              & \makecell{ToLD-Br\\(1000)~\citeyearpar{leite2020toxic}}                                   &                                                       &                                                         &                                                           \\ \midrule
% \multirow{12}{*}{\method-Es} & \multirow{12}{*}{Spanish}  & \multirow{12}{*}{Argentina, Mexico}     & Offensive detect             & \makecell{AMI\\(1000)~\citeyearpar{fersini2018overview}}                         & \makecell{MEX-A3T\\(1000)~\citeyearpar{alvarez2018overview}}                           & \makecell{OffendES\\(1000)~\citeyearpar{plaza2021offendes}}                                          &                                                           \\
%             &  &   & Hate detect                  & \makecell{HatEval 2019\\(1000)~\citeyearpar{basile2019semeval}}                              & \makecell{HaterNet\\(1000)~\citeyearpar{pereira2019detecting}}                                        &                                                         &                                                           \\
%             &  &   & Bias detect           & \makecell{DETOXIS\_stereotype\\(1000)~\citeyearpar{de2021ai}}                              &   \makecell{DETOXIS\_improper\\(1000)~\citeyearpar{de2021ai}}                                                 &                                                         &                                                           \\
%             &  &   & Abusive detect             & \makecell{DETOXIS\_abusive\\(1000)~\citeyearpar{de2021ai}}                              &   \makecell{DETOXIS\_mockery\\(1000)~\citeyearpar{de2021ai}}                                                      &                                                         &                                                           \\
%             &  &   & Aggressiveness detect & \makecell{DETOXIS\_aggressiveness\\(1000)~\citeyearpar{de2021ai}}                              &                                                       &                                                         &                                                           \\
%             &  &   & Stance detect               & \makecell{DETOXIS\_stance\\(1000)~\citeyearpar{de2021ai}}                              &                                                       &                                                         &                                                           \\ \midrule
% \multirow{8}{*}{\method-Tr} & \multirow{8}{*}{Turkish}  & \multirow{8}{*}{Turkey}     & Offensive detect             &  \makecell{SemEval-2020\\(3528)~\citeyearpar{zampieri2020semeval}} & \makecell{offenseCorpus\\(1000)~\citeyearpar{coltekin2020lrec}}                                   & \makecell{offenseKaggle\\(1000)~\citeyearpar{turkish-tweets}}                                     & \makecell{offenseKaggle\_2\\(1000)~\citeyearpar{turkish-offensive-language-detection}}                                    \\
%             &  &   & Abusive detect              & \makecell{ATC\\(1000)~\citeyearpar{karayiugit2021detecting}}                                       &                                                       &                                                         &                                                           \\
%             &  &   & Spam detect & \makecell{Turkish Spam\\(825)~\citeyearpar{misc_turkish_spam_v01_530}}                               &                                                       &                                                         &                                                           \\
%             &  &   & Fine-grained offensive detect & \makecell{offenseCorpus\\(1000)~\citeyearpar{coltekin2020lrec}}                             &                                                       &                                                         &                                                           \\
%            &                              &                                                 &                                                       &    
% &
\\ \bottomrule                                                 
\end{tabular}
}
\end{table*}


==> tables/case-study/tb-case-arabic.tex <==
\begin{table*}[htbp]
\caption{Case study on Arabic Culture.}
\label{tb-case-arabic}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{p{5cm}|p{15cm}}
\toprule
Question & Is the following sentence offensive? 
\begin{Arabic}
 مالك يا اوبا يا حبيبي ؟؟ ما تركز يابني
\end{Arabic}\\\midrule
Response from ChatGPT & 
 The sentence
\begin{Arabic}
    مالك يا اوبا يا حبيبي ؟؟ ما تركز يابني
\end{Arabic} can be considered offensive depending on the context and the relationship between the speaker and the listener. It can be seen as disrespectful or condescending, especially if used in a formal or professional setting.\\ \midrule
Response from \method-Ar & No, the sentence is not offensive. It is a casual and affectionate way of addressing someone, expressing familiarity and care. \\ \midrule \midrule

Question & Is the following sentence offensive? 
\begin{Arabic}
 يا حزني يا ولاه الموضوع بجا شين علاولة 
\end{Arabic}\\\midrule
Response from ChatGPT & As an AI language model, I don't have personal emotions, but I can analyze the sentence for you. The given sentence includes informal language and the use of emojis. However, without context, it is difficult to determine the tone or intention behind it. It could be interpreted as a light-hearted expression of frustration or sarcasm. Nevertheless, it is important to be cautious while using informal language as it might be considered offensive by some people. \\ \midrule
Response from \method-Ar & No, the sentence is not offensive. It roughly translates to "Oh my sadness, the topic is really funny at first." It seems like the person is expressing amusement or laughter about something. \\ \bottomrule
\end{tabular}
}

\end{table*}

==> tables/case-study/tb-case-english.tex <==
\begin{table*}[htbp]
\caption{Case study on English Culture.}
\label{tb-case-english}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{p{5cm}|p{15cm}}
\toprule
Question & Does tthe following sentence have hate speech? : @user @user even called country shithole people shithole people. sad. \\\midrule
Response from ChatGPT & The sentence you provided does not contain hate speech itself, but it does refer to derogatory language and offensive sentiments. It is important to promote respectful and inclusive communication. \\ \midrule
Response from \method-En &  Yes, the sentence contains hate speech as it includes derogatory language and insults towards a particular country and its people. \\ \midrule \midrule

Question & Does tthe following sentence have hate speech? : also believes slaves immigrants. he's fool disgrace injustices done his gop white peop @url \\\midrule
Response from ChatGPT & I'm sorry, but I cannot assess the content of a specific URL or webpage. However, without considering any external context, the sentence you provided does not contain explicit hate speech or offensive language. \\ \midrule
Response from \method-En &  Yes, the following sentence contains hate speech and offensive language. \\ \bottomrule
\end{tabular}
}

\end{table*}

==> tables/case-study/tb-case-germany.tex <==
\begin{table*}[htbp]
\caption{Case study on German Culture.}
\label{tb-case-germany}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{p{5cm}|p{15cm}}
\toprule
Question & Does the following sentence have hate speech? : War das Wochenende im Ruhrpott unterwegs. Überall schwangere, muslimische Frauen mit einem Rattenschwanz an Kindern \#Islamisierung\\\midrule
Response from ChatGPT & As an AI language model, I can provide you with an analysis of the sentence you provided. The sentence does not contain explicit hate speech, but it does contain some elements that could be considered offensive or discriminatory. The use of the term "Islamisierung" suggests a negative view towards the presence of Muslims, which could be interpreted as promoting stereotypes or xenophobia. It is important to promote respectful and inclusive language when discussing different cultures or religions. \\ \midrule
Response from \method-De & Yes, the sentence contains hate speech as it generalizes and stigmatizes pregnant Muslim women and implies negative intentions regarding their presence in the Ruhrpott region. \\ \midrule \midrule

Question & Does the following sentence have hate speech? : In diesem Moment wird die Ernst-Grube-Halle endlich geräumt \#leipzig \#npd \#jn \#Legida \#RefugeesNotWelcome \\\midrule
Response from ChatGPT & As an AI language model, I can provide you with an analysis of the sentence structure and content, but I cannot determine the intention or context behind it. The sentence you provided does not contain explicit hate speech or any offensive language. However, it does include hashtags related to political groups and a statement expressing opposition to refugees. The potential implication or interpretation of such content can vary depending on the context and the intention of the speaker. \\ \midrule
Response from \method-De & Yes, the sentence contains hate speech as it expresses a negative sentiment towards refugees. \\ \bottomrule
\end{tabular}
}

\end{table*}

==> tables/case-study/tb-case-spanish.tex <==
\begin{table*}[htbp]
\caption{Case study on Spanish Culture.}
\label{tb-case-spanish}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{p{5cm}|p{15cm}}
\toprule
Question & Is the following sentence offensive? @dsilvao Más que seguro que muchos nacieron producto de acoso y hasta violación. Personalmente, nunca he tenido problemas para conquistar sin recurrir a la intimidación. \\\midrule
Response from ChatGPT & As an AI language model, it is my duty to provide objective information. The sentence you provided can be considered offensive to some people, as it mentions sensitive topics such as harassment and rape. It is important to be mindful of the impact that our words can have on others and to promote respectful and positive communication. \\ \midrule
Response from \method-Es & The first part of the sentence is not offensive, as it states that it is very likely that many people were born as a result of harassment and even rape. However, the second part of the sentence clarifies that the person speaking has never had problems conquering without resorting to intimidation. \\ \midrule \midrule

Question & Is the following sentence offensive? Ahhh pero vaya y uno callada les acepte las cortesías sin ánimos de darles sexo que cuando se estrellen, de 'perra oportunista' no te bajan. \\\midrule
Response from ChatGPT & As an AI language model, I can tell you that the sentence you provided contains offensive language and derogatory terms. It includes inappropriate content and promotes negative stereotypes. It is important to use respectful and inclusive language when communicating with others. \\ \midrule
Response from \method-Es & No, the sentence is not offensive. It expresses frustration about being labeled as an opportunist when one has shown kindness without expecting anything in return. \\ \bottomrule
\end{tabular}
}

\end{table*}

==> tables/examples/tb-example-1.tex <==
\begin{table}[]
\caption{An example that can not be clearly answered by LLMs}
\label{tb-example-1}
\centering
\resizebox{1\textwidth}{!}{
% \begin{tabular}{ll}
\begin{tabular}{c m{20cm}}
\toprule
\multicolumn{1}{c}{Input}    & \multicolumn{1}{c}{On this card are three basic kinds of attitudes concerning the society we live in. Please choose the one which best describes your own opinion?** 1 The entire way our society is organized must be radically changed by revolutionary action 2 Our society must be gradually improved by reforms 3 Our present society must be valiantly defended against all subversive forces} \\
\multicolumn{1}{c}{Response} & \multicolumn{1}{c}{As an AI language model, I don't have personal opinions. However, individuals may choose any of the options based on their beliefs and values. It's important to note that each attitude represents a different perspective on societal change: 1. **Revolutionary Action:** This attitude suggests a belief in the necessity of fundamental, drastic change to the societal structure. It advocates for overthrowing existing systems and instituting new ones. 2. **Gradual Reform:** This viewpoint holds that change should occur incrementally through reform efforts within the existing societal framework. It seeks to address issues within the system without completely dismantling it. 3. **Defense of Present Society:** This stance prioritizes the preservation and protection of the current societal structure against perceived threats or challenges. It emphasizes maintaining stability and resisting changes that may disrupt the status quo. Individuals may align with any of these attitudes based on their assessment of societal issues and their preferred methods of addressing them.} \\
\bottomrule  
\end{tabular}
}
\end{table}

==> tables/examples/tb-example-2.tex <==
\begin{table}[]
\caption{An example that can not be clearly answered by LLMs}
\label{tb-example-2}
\centering
% \begin{tabular}{ll}
\begin{tabular}{c|p{10cm}}
\toprule
\multicolumn{1}{c}{Input}    & \multicolumn{1}{c}{Taking all things together, would you say you are** 1 Very happy 2 Rather happy 3 Not very happy 4 Not at all happy} \\
\multicolumn{1}{c}{Response} & \multicolumn{1}{c}{As an artificial intelligence, I don't have feelings or emotions, so I can't experience happiness or any other emotions. Therefore, I cannot answer this question based on personal experience. However, I can provide information or guidance on how to assess one's own happiness or well-being if that's helpful.} \\
\bottomrule  
\end{tabular}
\end{table}

==> tables/tb-CultureLLMs.tex <==
\begin{table}[]
\label{tb-CultureLLMs}
\caption{Each CultureLLM has specific targeted culture, and is fine-tuned by people's opinions from corresponding countries. This table shows the details on our CultureLLMs concerning targeted culture, country data for fine-tuning, and culture's main language.}
\resizebox{.5\textwidth}{!}{
\begin{tabular}{llll}
\toprule
\multicolumn{1}{c}{CultureLLM}    & \multicolumn{1}{c}{Targeted Culture} & \multicolumn{1}{c}{Country}              & \multicolumn{1}{c}{Main Language} \\ \midrule
\multicolumn{1}{c}{ArabicLLM}     & \multicolumn{1}{c}{Arabic}           & \multicolumn{1}{c}{Iraq and Jordan}      & \multicolumn{1}{c}{Arabic}        \\
\multicolumn{1}{c}{BengaliLLM}    & \multicolumn{1}{c}{Bengali}          & \multicolumn{1}{c}{Bangladesh}           & \multicolumn{1}{c}{Bengali}       \\
\multicolumn{1}{c}{ChineseLLM}    & \multicolumn{1}{c}{Chinese}          & \multicolumn{1}{c}{China}                & \multicolumn{1}{c}{Chinese}       \\
\multicolumn{1}{c}{EnglishLLM}    & \multicolumn{1}{c}{English}          & \multicolumn{1}{c}{United States}        & \multicolumn{1}{c}{English}       \\
\multicolumn{1}{c}{GermanLLM}     & \multicolumn{1}{c}{German}           & \multicolumn{1}{c}{Germany}              & \multicolumn{1}{c}{German}        \\
\multicolumn{1}{c}{KoreanLLM}     & \multicolumn{1}{c}{Korean}           & \multicolumn{1}{c}{South Korea}          & \multicolumn{1}{c}{Korean}        \\
\multicolumn{1}{c}{PortugueseLLM} & \multicolumn{1}{c}{Portuguese}       & \multicolumn{1}{c}{Brazil}               & \multicolumn{1}{c}{Portuguese}    \\
\multicolumn{1}{c}{SpanishLLM}    & \multicolumn{1}{c}{Spanish}          & \multicolumn{1}{c}{Argentina and Mexico} & \multicolumn{1}{c}{Spanish}       \\
\multicolumn{1}{c}{TurkishLLM}    & \multicolumn{1}{c}{Turkish}          & \multicolumn{1}{c}{Turkey}               & \multicolumn{1}{c}{Turkish}       \\     \bottomrule              
\end{tabular}
}
\end{table}

==> tables/tb-compare-ko.tex <==
\begin{table}[]
\caption{Comparative analysis with other Korean models}
\label{tb-compare-ko}
\centering
\begin{tabular}{lllllll}
\toprule
\multicolumn{1}{c}{Model}          & \multicolumn{1}{c}{abusive\_1} & \multicolumn{1}{c}{abusive\_2} & \multicolumn{1}{c}{abusive\_3} & \multicolumn{1}{c}{hate\_1} & \multicolumn{1}{c}{hate\_2} & \multicolumn{1}{c}{hate\_3} \\ \midrule
\multicolumn{1}{c}{\method-Ko} & \multicolumn{1}{c}{0.779}      & \multicolumn{1}{c}{0.599}      & \multicolumn{1}{c}{0.613}      & \multicolumn{1}{c}{0.747}   & \multicolumn{1}{c}{0.686}   & \multicolumn{1}{c}{0.570}   \\
\multicolumn{1}{c}{CultureLLM-One} & \multicolumn{1}{c}{0.703}      & \multicolumn{1}{c}{0.582}      & \multicolumn{1}{c}{0.572}      & \multicolumn{1}{c}{0.563}   & \multicolumn{1}{c}{0.526}   & \multicolumn{1}{c}{0.481}   \\
\multicolumn{1}{c}{SeaLLM}         & \multicolumn{1}{c}{0.596}      & \multicolumn{1}{c}{0.428}      & \multicolumn{1}{c}{0.547}      & \multicolumn{1}{c}{0.378}   & \multicolumn{1}{c}{0.545}   & \multicolumn{1}{c}{0.404}   \\ \bottomrule               
\end{tabular}
\end{table}
